The quark susceptibility in a generalized dynamical quasiparticle model

The quark susceptibility $\chi_q$ at zero and finite quark chemical potential provides a critical benchmark to determine the quark-gluon-plasma (QGP) degrees of freedom in relation to the results from lattice QCD (lQCD) in addition to the equation of state and transport coefficients. Here we extend the familiar dynamical-quasiparticle model (DQPM) to partonic propagators that explicitly depend on the three-momentum with respect to the partonic medium at rest in order to match perturbative QCD (pQCD) at high momenta. Within the extended dynamical-quasi-particle model (DQPM$^*$) we reproduce simultaneously the lQCD results for the quark number density and susceptibility and the QGP pressure at zero and finite (but small) chemical potential $\mu_q$. The shear viscosity $\eta$ and the electric conductivity $\sigma_e$ from the extended quasiparticle model (DQPM$^*$) also turn out in close agreement with lattice results for $\mu_q$ =0. The DQPM$^*$, furthermore, allows to evaluate the momentum $p$, temperature $T$ and chemical potential $\mu_q$ dependencies of the partonic degrees of freedom also for larger $\mu_q$ which are mandatory for transport studies of heavy-ion collisions in the regime 5 GeV $< \sqrt{s_{NN}} <$ 10 GeV.

==> acknowledgment.tex <==
\vspace{-3mm}
\section*{Acknowledgment}
\vskip -3mm

 H. Berrehrah acknowledges the financial support through DFG and the ``HIC for FAIR'' framework of the ``LOEWE'' program. The computational resources have been provided by the LOEWE-CSC.

% The authors acknowledge valuable discussions with R. Marty and O. Linnyk, and the financial support through the `HIC for FAIR' framework of the `LOEWE' program.

